Variability and Evolution in Systems of Systems

In this position paper (1) we discuss two particular aspects of Systems of Systems, i.e., variability and evolution. (2) We argue that concepts from Product Line Engineering and Software Evolution are relevant to Systems of Systems Engineering. (3) Conversely, concepts from Systems of Systems Engineering can be helpful in Product Line Engineering and Software Evolution. Hence, we argue that an exchange of concepts between the disciplines would be beneficial.

==> eptcsdata.tex <==
\providecommand{\firstpage}{8}
\providecommand{\publicationstatus}{Larsen, Legay, Nyman (Eds.): 1st Workshop on \\
Advances in Systems of Systems (AiSoS 2013)\\
EPTCS 133, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.133.2}{10.4204/EPTCS.133.2}}
\pdfoutput=1

